Online Hybrid Lightweight Representations Learning: Its Application to Visual Tracking

This paper presents a novel hybrid representation learning framework for streaming data, where an image frame in a video is modeled by an ensemble of two distinct deep neural networks; one is a low-bit quantized network and the other is a lightweight full-precision network. The former learns coarse primary information with low cost while the latter conveys residual information for high fidelity to original representations. The proposed parallel architecture is effective to maintain complementary information since fixed-point arithmetic can be utilized in the quantized network and the lightweight model provides precise representations given by a compact channel-pruned network. We incorporate the hybrid representation technique into an online visual tracking task, where deep neural networks need to handle temporal variations of target appearances in real-time. Compared to the state-of-the-art real-time trackers based on conventional deep neural networks, our tracking algorithm demonstrates competitive accuracy on the standard benchmarks with a small fraction of computational cost and memory footprint.

==> sections/__latexindent_temp.tex <==
% !TEX root = ../main.tex
\section{Online Hybrid Representation Learning}
%\section{Online Representation Learning using Quantized and Pruned Networks}
\label{sec:online}


This section describes the proposed deep neural network architecture with the offline and online training strategies for robust hybrid feature representations.


\subsection{Overview of Hybrid Representation}
%\subsection{Overview}
\label{sub:overview}
% Our main idea is to enhance the expressiveness of the convolutional feature extractor by exploiting an ensemble of two lightweight deep neural networks, a quantized network (Section~\ref{sub:low-bit}) and a channel-pruned network (Section~\ref{sub:channel}). 
Our goal is to enhance the quality of representations using an ensemble of two lightweight deep neural networks obtained from quantization and channel pruning.
%The quantization network is responsible for feature encoding of primary information while the channel-pruned model enhances the learned representations with high-precision residual information. 
The quantized network is responsible for feature encoding of the primary time-invariant information while the channel-pruned model covers high-precision time-varing residual information. 
%Before discussing the technical details, we define the notations and the expressions used in this paper. 

Given an input image $A_0$, the standard convolutional neural network (CNN) learns a feature extractor $\mathtt{f}_\textrm{conv}(\cdot ; \cdot)$ and estimates a feature map $A_\textrm{conv}$ as follows:
%
\begin{equation} \label{formula:conv_layer}
    A_\textrm{conv} \equiv A_{N_l}  = \mathtt{f}_\textrm{conv} (A_{0}; \mathcal{W}_\textrm{conv}),
\end{equation}
where $\mathcal{W}_\textrm{conv} = \{ W_1, ..., W_{N_l}\}$ is a collection of convolutional filters throughout the $N_l$ layers.
%
In the $i^\text{th}$ intermediate layer, we apply a convolution with auxiliary operations and derive a feature map, which is given by
%
\begin{equation}
A_{i} = \sigma(A_{i-1} * W_{i} ),
\end{equation}
%
where $\sigma(\cdot)$ denotes a non-linear activation function and $*$ indicates the convolution operator. 
%By representing the entire convolution layers as a feature extractor function $\mathtt{f}_\textrm{conv}(\cdot ; \cdot)$, the relationship between input and output activation is described as
%
Contrary to the conventional CNNs, our framework utilizes two networks in parallel, a quantized network $\mathtt{f}^q (\cdot ; \cdot)$ and a channel-pruned network $\mathtt{f^p} (\cdot ; \cdot)$,
%Denote by $\mathcal{W}^q = \{ W^q_l \}_{l=1:N_l}$ and $\mathcal{W}^p = \{ W^p_l \}_{l=1:N_l}$ the $N_b$-bit quantized parameters of the backbone network and the channel-pruned parameters in the residual branch, respectively.
which generate outputs respectively as 
%
\begin{align}
    A^\textrm{q} = \mathtt{f}^q(A_0; \mathcal{W}^\textrm{q}), ~~~ \mathcal{W}^\textrm{q}=\{ W_1^\textrm{q},...,W_{N_l}^\textrm{q} \}, \\
    A^\textrm{p} = \mathtt{f}^p(A_0; \mathcal{W}^\textrm{p}),  ~~~ \mathcal{W}^\textrm{p}=\{ W_1^\textrm{p},...,W_{N_l}^\textrm{p} \}.
\end{align}
Then, the proposed hybrid representation, $A^\textrm{h}$, is given by the sum of two outputs as follows:
%%%%%%%%
\begin{equation}
A^\textrm{h} = A^q + A^p \nonumber = \mathtt{f}^\textrm{q}(A_0; \mathcal{W}^q) + \mathtt{f}^\textrm{p}(A_0; \mathcal{W}^p). 
\end{equation}
%%%%%%%%
%
We can train prediction networks of arbitrary tasks followed by the feature extraction.
Note that the hybrid representation is also utilized in the prediction networks; channel pruning is applied to all layers of the prediction networks while low-bit quantization is partially applied to the activation quantization.

\subsection{Low-Bit Quantization of Primary Network}
\label{sub:low-bit}
To maximize the benefit of the reduced precision network, 
we quantize both model parameters %, $\mathcal{W}_\textrm{conv} = \{W_{l}\}_{l=1:N_l}$, 
and activations %, $\mathcal{A} = \{A_l \}_{l=1:N_l}$, 
in all $N_l$ layers.
%We adopt the quantization method proposed in \cite{jung2019learning} except for the input of the first convolution layer and the output of the last convolution layer. 
We adopt the quantization method proposed in \cite{jung2019learning}, and introduce the additional regularization loss terms to the quantized data for fast and stable training.
%In addition to the quantization algorithm,  we also introduce the additional regularization loss terms to the quantized data for fast and stable training.
%In the rest of this subsection, we describe the quantization method and normalization technique employed in our work.

\subsubsection{Weight Quantization}

The weight quantization function $Q_W^l(\cdot): w_l \rightarrow w^q_l$ is composed of two steps.
First, the weights are linearly transformed to $[-1,1]$ by the learnable parameters $c^l_W$ and $d^l_W$, which define the center and the width of the quantization interval, respectively.
% First, the weights are linearly transformed to $[-1,1]$ by the learnable parameters $\{ c^l_W, d^l_W\}$, which define the center and the width of the quantization interval. 
Only the weight values within the interval $[c_W^l-d_W^l, c_W^l+d_W^l]$ are quantized while the rests are clamped.
The formal definition of the first step is given by
%
\begin{equation}
\hat{w}_{l} =
\begin{cases}
\mathtt{sign}(w_{l}) & \text{if $|w_{l}| > c^l_{W} + d^l_{W}$ } \\
0 & \text{if $|w_{l}| < c^l_{W} - d^l_{W}$ } \\
\mathtt{sign}(w_{l}) \cdot (\alpha^l_{W} |w_{l}| + \beta^l_{W}) & \text{otherwise},
%\texttt{sign}(w_{l}) \cdot (\alpha^l_{W} |w_{l}| + \beta^l_{W})^{\gamma^l_{W}} & \text{otherwise},
\end{cases}
\label{eq:quantization_w}
\end{equation}
%
where $\mathtt{sign}(\cdot) \in \{-1, 1\}$ means the sign of an input, $\alpha^l_{W} = 0.5/d^l_{W}$, and $\beta^l_{W}= -0.5 c^l_{W} / d^l_{W} + 0.5$. 
Second, the normalized weights are discretized as 
%by the element-wise rounding function, $\mathtt{round}(\cdot)$, as $W^q_l = \mathtt{round}(\hat{W}_l \cdot (2^{N_b-1}-1))$, 
%
\begin{equation}
W^q_l = \mathtt{round}(\hat{W}_l \cdot (2^{N_b-1}-1)),
\label{eq:quantize_w}
\end{equation}
%
where $\mathtt{round}(\cdot)$ denotes the element-wise rounding and $N_b$ is the bit-width, leading to $(2^{N_b}-1)$ quantization levels. % Note that \eqref{eq:quantize_w} quantizes the absolute values of weights using $N_b-1$ bits and one bit is reserved for the sign of each weight.



%\ilchae{[Explanation of acitivation quantization]}
\subsubsection{Activation Quantization}
% The activation quantization function $Q_A^l(\cdot): a_l \rightarrow a^q_l$ also has two steps.
% First, all activations $a_l \in A_l$ in the $l^\text{th}$ layer are transformed to $\hat{a}_l \in \hat{A}_l$, which is in the range of $[0, 1]$ as in the following equation:
Similarly, the activation quantization function $Q_A^l(\cdot): a_l \rightarrow a^q_l$ has transformation and round steps.
First, the activations $a_l \in A_l$ in the $l^\text{th}$ layer are linearly transformed to the values in $[0, 1]$ as follows:
%
\begin{equation}
\hat{a}_l = 
\begin{cases}
1 & \text{if $a_l > c^l_{A} + d^l_{A}$ } \\
0 & \text{if $a_l < c^l_{A} - d^l_{A}$ } \\
\alpha^{l}_{A} A_l + \beta^{l}_{A} & \text{otherwise}
\end{cases},
\label{eq:quantization_a}
\end{equation}
%
where $\alpha^l_{A} = 0.5/d^l_{A}$ and $\beta^l_{A}= -0.5 c^l_{A} / d^l_{A} + 0.5$. 
The quantization interval is defined by the learnable parameters for its center ($c^l_A$) and width ($d^l_A$). 
We assume that the activations are non-negative due to the ReLU function.  
%In other words, $[c^l_{A} - d^l_{A}, c^l_{A} + d^l_{A}]$ is transformed linearly to $[0, 1]$.
The final quantized output $A^q_l$ is obtained by applying the rounding function to the individual elements in $\hat{A}_l$.
%which is given by  $A^q_l =  \mathtt{round}(\hat{A}_l \cdot (2^{N_b}-1))$.  
%
\begin{equation}
A^q_l =  \mathtt{round}(\hat{A}_l \cdot (2^{N_b}-1)).
\label{eq:quantize}
\end{equation}
%We define whole matrix-wise transformation as $\mathtt{trans}^l_A() \textrm{ s.t. }  \hat{A}_l=\mathtt{trans}^l_A(A_l)$.
%

\subsubsection{Operation of Quantization Network}
% To reduce the computational cost, we apply both the activation and weight quantization at the same time during the convolution operation. 
%To reduce the computational cost of the neural network, both the weight quantization function $Q_W^l(\cdot)$ and the activation quantization function $Q_A^l(\cdot)$ are applied to the convolution layer.
%Specifically, the output from each convolutional layer is given by
The output from each convolutional layer is now given by $A_{l+1} = \sigma (Q_A^l(A_l) * Q_W^{l+1}(W_{l+1}) ),$
%% 
%\begin{equation}
%A_{l+1} = \sigma (Q_A^l(A_l) * Q_W^{l+1}(W_{l+1}) ),
%\end{equation}
%
where the standard convolution operation is replaced by a hardware-friendly fixed-point operation for additional acceleration.
By applying the quantization to the whole network, the representation of the final convolutional layer is denoted by %$A^q \equiv \mathtt{f}^q(A_0; \mathcal{W}^q)$,
%%
\begin{equation}
A^q=\mathtt{f}^q(A_0; \mathcal{W}^q),
\end{equation}
%
where $\mathtt{f}^q (\cdot ; \cdot)$ is the feature extraction network via the quantization of both weights and activations.
%
%
\iffalse
{\color{blue}[To Delete]
Figure~\ref{fig:quantization} illustrates the framework of quantizing each layer's input activation.
%%%%%%%%%%%%%%%
\begin{figure}
	\centering
		\includegraphics[width=0.98\linewidth]{figs/quantization.pdf}
		\vspace{-0.1cm}
	\caption{Overall framework of quantizing $l^\textrm{th}$ layer's input activation. By observing input activation set $A_l$, we linearly transform the activations within quantization interval ($c^l_A - d^l_A,c^l_A + d^l_A$) to be locate in [0,1] (\textbf{Trans}). Note that the values lower than $c^l_A - d^l_A$ are pruned to 0 while the values upper than $c^l_A + d^l_A$ are clamped to 1. After that, we obtain quantized activations $A^q_l = \mathtt{round}(\hat{A}_l \cdot (2^N_b -1))$ (\textbf{Quantize}).} 
	\label{fig:quantization}
\end{figure} 
% %%%%%%%%%%%%%%%%
}
\fi

\subsubsection{Training Quantization Networks with Normalization}
We now present our training scheme for robust and stable quantization. 
In particular, we discuss a novel regularization loss for quantization, $\mathcal{L}_\textrm{quant}$, which is divided into weight and activation normalization losses as %$\mathcal{L}_\textrm{quant} = \mathcal{L}_\textrm{qW} + \mathcal{L}_\textrm{qA}$.
%%
\begin{align}
	\mathcal{L}_\textrm{quant} = \mathcal{L}_\textrm{qW} + \mathcal{L}_\textrm{qA}.
\end{align}
%%
%We discuss each of two loss terms in the following.

\iffalse
{\color{blue}
%%%%%%%%%%%%%%%%
\begin{figure}
	\centering
		\includegraphics[width=0.95\linewidth]{figs/L_qw.pdf}
 	\caption{Clipping model parameters using the learned interval leads to losing details in the quantized representations and makes the optimization procedure unstable. To alleviate the limitation, we propose a simple but effective regularizer, $\mathcal{L}_\textrm{qW}$,encouraging a majority of parameters to be located within a certain range.} 
	\label{fig:lqw}
\end{figure} 
%%%%%%%%%%%%%%%%
}
\fi

%\ilchae{[weight normalization with standard distribution]}
\paragraph{Weight normalization.}
Clipping model parameters using the learned interval $[c_W^l - d_W^l, c_W^l + d_W^l]$ leads to error in the quantized representations and makes the optimization procedure unstable.
%It turns out that the final accuracy is sensitive to the initialization of $(c^l_W, d^l_W, \gamma_W^l)$, which is aggravated when the quantization is based on lower bits\footnote{When we attempted the network quantization based on \cite{jung2019learning}, 5-bit quantization was much easier than 4-bit counterpart.}.
It turns out that the final accuracy is sensitive to the initialization of $\{c^l_W, d^l_W\}$, especially with a lower bit-width.  %\footnote{When we tested network quantization based on \cite{jung2019learning}, 5-bit task was much easier than 4-bit counterpart.}.
To alleviate the limitation, we propose a simple but effective regularizer, $\mathcal{L}_\textrm{qW}$, enforcing a majority of parameters to be located within a certain range, which is given by
%
\begin{align}
    \mathcal{L}_\textrm{qW}(\mathcal{W}_\textrm{conv}) = \sum^{N_l}_{i=1} \begin{pmatrix}\left(\mathtt{avg}({ \alpha^i_W |W_{i}| +\beta^i_W }) - \mu_0\right)^2 \nonumber \\  +\left(\mathtt{std}({  \alpha^i_W |W_{i} | + \beta^i_W })-\sigma_0\right)^2 \end{pmatrix} ,
\end{align}
%\ilchae{shoud fix the regularizer. Motivation(regularizing the range containing the most of parameters and activateion) is not changed.}
%
where $\mathtt{avg}(\cdot)$ and $\mathtt{std}(\cdot)$ denote mean and standard deviation of all entries in their input matrices, respectively, $| \cdot |$ returns an absolute value matrix of the same size to its input, and $(\mu_0, \sigma_0)$ are hyperparameters for desirable mean and standard deviation values.
% By selecting the proper values in the range of $( 0,1 )$ for both $\mu_0$ and $\sigma_0$, the regularizer enforces model parameters to move into the range.
% By enforcing the distribution of model parameters using this regularizer, it is possible to identify more appropriate parameters ($c^l_W, d^l_W$) and train the network more efficiently and stably.
The proposed regularizer encourages the transformed model parameters to be in $[0,1]$ and reduces the error resulting from the clamping process.
Note that it allows the quantized network to identify more appropriate parameters ($c^l_W, d^l_W$) and undergo more stable optimization.

\iffalse
{\color{blue} [To Delete]
Figure~\ref{fig:lqw} illustrate the effect of the weight normalization briefly.
}
\fi

\paragraph{Activation normalization.}
\label{paragraph:act_norm}
Clipping activations outside of the interval $[c^l_\textrm{A}-d^l_\textrm{A}, c^l_\textrm{A}+d^l_\textrm{A}]$ incurs critical information loss in practice.
%To mitigate this issue, we employ a similar technique with weight normalization and define the following regularization loss term $\mathcal{L}_\textrm{qA}$:
To mitigate this issue, we define the following regularization loss term $\mathcal{L}_\textrm{qA}$:
%
\begin{align}
%    \mathcal{L}_\textrm{qA}(A^\textrm{bn}) = \sum^{N_l}_{i=1} \left[ \mathtt{avg}(A_i^\textrm{bn}) + 2 \cdot \mathtt{std}(A_i^\textrm{bn}) - \mathtt{UB} \right]_{+} \nonumber   +  \left[ \sigma_i - \mathtt{std}(A_i^\textrm{bn}) \right]_{+} +  \left[ \mu_i - \mathtt{avg}(A_i^\textrm{bn}) \right]_{+},
    %\mathcal{L}_\textrm{qA} & (A^\textrm{bn}) =  \\
    %& \sum^{N_l}_{i=1} \left[ \mathtt{avg}(A_i^\textrm{bn}) + 2 \cdot \mathtt{std}(A_i^\textrm{bn}) - (c^l_\textrm{A}+d^l_\textrm{A}) \right]_{+} \hspace{-0.1cm}  +  \left[ \sigma_i - \mathtt{std}(A_i^\textrm{bn}) \right]_{+} \hspace{-0.1cm} + \left[ \mu_i - \mathtt{avg}(A_i^\textrm{bn}) \right]_{+}, \nonumber
    \mathcal{L}_\textrm{qA} & (A^\textrm{bn}) =  \sum^{N_l}_{i=1}\{ \left[ \mathtt{avg}(A_i^\textrm{bn}) + 2 \cdot \mathtt{std}(A_i^\textrm{bn}) - (c^l_\textrm{A}+d^l_\textrm{A}) \right]_{+}  \nonumber \\ &+  \left[ \sigma_i - \mathtt{std}(A_i^\textrm{bn}) \right]_{+}  + \left[ \mu_i - \mathtt{avg}(A_i^\textrm{bn}) \right]_{+}\}, 
\end{align}
%
where $A^\textrm{bn}=\{  A_i^\textrm{bn}  \}_{i=1}^{N_l}$ is a set of activations after batch normalization and $\left[ \cdot \right]_+$ denotes the ReLU function.
Note that $\sigma_i$ and $\mu_i$ are determined by combination of current quantization interval parameters ($c^l_A, d^l_A$).
Assuming that the activation $A_i^\textrm{bn}$ follows a Gaussian distribution, the regularization loss enforces the activations larger than the mean of the Gaussian and lower than $\mathtt{avg}(A^\textrm{bn}_i)+2\cdot \mathtt{std}(A^\textrm{bn}_i)$ to be within the active range.
Statistically speaking, it implies that almost 96$\%$ of positive values are trained to be located in the active range.
%%
%%
\iffalse
{\color{blue}[To Delete]
Figure~\ref{fig:lqa} illustrate the effect of the activation normalization briefly.
%%%%%%%%%%%%%%%
 \begin{figure}
 	\centering
 		\includegraphics[width=0.95\linewidth]{figs/L_qa.pdf}
 	\caption{Clipping activations outside of the interval incurs critical information loss in practice. To mitigate this issue, we employ a similar technique with weight normalization and define the regularization loss term $\mathcal{L}_\textrm{qA}$.} 
 	\label{fig:lqa}
 \end{figure} 
%%%%%%%%%%%%%%%%
}
\fi


%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
	\centering
		\includegraphics[width=0.9\linewidth]{figs/framework.pdf}
		\vspace{-0.1cm}
	\caption{Overall framework of our algorithm. We train hybrid representation for both low-bit quantized network ($\mathtt{f}^q$) and lightweight full precision network ($\mathtt{f}^p$) on pretraining time while only light weight network is fine-tuned in test phase.
	Red arrow denotes the gradient backpropagation of full precision network in online model update and pretraining while blue arrow denotes the backpropagation in pretraining. 
%Note that $\mathcal{L}_\textrm{track}$ denotes the original objective of baseline trackers.
}
	\label{fig:overall_framework}
	%\vspace{-0.2cm}
\end{figure*} 
%%%%%%%%%%%%%%%%%%%

\subsection{Channel Pruning of Residual Network}
\label{sub:channel}

%\ilchae{[Explanation of gumbel softmax application to model channel pruning]}
We propose a stochastic channel pruning algorithm using a Gumbel-softmax trick to generate discrete mask samples from the model with a continuous output space.
Our algorithm learns a set of channel selection probability vectors, $\{ \mathbf{b}_1, ..., \mathbf{b}_{N_{l}}\}$, in each layer, where $\mathbf{b}_l$ indicates which channel is likely to be sampled in the $l^\textrm{th}$ layer.
%Note that we employ channel pruning algorithm for all $N_{pl}$ layers of whole model including $N_l$ layers of backbone CNN.
% aaaaaaabbbbbccccaaaaaaabbbbbccccaaaaaaabbbbbccccaaaaaaabbbbbcccc
By employing the Gumbel-softmax trick introduced in \cite{jang2016categorical}, $\mathbf{b}_l$ generates discrete channel selection mask $\mathbf{M}_{l}$ as follows:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\label{formula:pruning}
    %\begin{matrix}
\bar{\mathbf{M}}_l[i] & = \frac{\exp\left( \frac{g_i + \log (\mathbf{b}_l[i])}{\tau} \right) }{ \exp \left( \frac{g_i + \log (\mathbf{b}_l[i])}{\tau} \right) + \exp \left( \frac{g_i + \log(1- \mathbf{b}_l[i])}{\tau} \right) }, \nonumber \\
\mathbf{M}_l[i] & = \mathtt{round}(\bar{\mathbf{M}}_l[i]) , 
    %\end{matrix}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $g_i$ represents a random noise sample from Gumbel distribution, and $\tau$ denotes a temperature.
%where $g_i$ represents a random noise sample from Gumbel distribution, $\mathtt{Gumbel}(0,1)$, and $\tau$ denotes a temperature.
We apply the straight-through Gumbel estimator for gradient approximation in backpropagation similarly to \cite{jang2016categorical}.
In the forward pass of training, we apply the pruning mask $M_{l}$ to the output activation  $A^p_l$ in the $l^\textrm{th}$ layer, which is given by
%
\begin{equation}
A^p_{l} = \sigma ( A^p_{l-1} * W^p_{l} ) \odot \mathbf{M}_{l},  \quad l =1 \dots N_{l}
\end{equation}
%
where $\odot$ denotes an channel-wise multiplication.
%where $l =1 \dots N_{pl}$ and $\odot$ denotes an channel-wise multiplication.
Then, the representation of the final convolution layer is obtained by applying the channel pruning network $\mathtt{f}^p(\cdot ; \cdot)$, as follows: $A^p =  \mathtt{f}^p(A_0; \mathcal{W}^p)$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{align}
%	A^p &=  \mathtt{f}^p(A_0; \mathcal{W}^p),
%\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%where $ \mathcal{W}^p = \{ W^p_l \}_{l=1}^{N_{pl}}$ is the set of convolution parameters in the pruned network.
Note that a channel with a selection probability lower than the threshold is removed at testing.
For training, the channel selection probabilities $ \{ \mathbf{b}_l \}^{N_{l}}_{l=1}$ are learned by minimizing the following loss term %$\mathcal{L}_\textrm{prune}= \sum^{N_{l}}_{l=1} ||\mathbf{M}_{l}||_1$, 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
   \mathcal{L}_\textrm{prune} = \sum^{N_{l}}_{l=1} ||\mathbf{M}_{l}||_1.
 %   %\mathcal{L}_\textrm{pW} = \sum^{N_l}_{l=2} ||\mathbf{M}_{l}||_1.
\end{align}
where the number of active channels is penalized.


% \iffalse
% Figure~\ref{fig:pruning} briefly shows the layerwise pruning scenario.
% %%%%%%%%%%%%%%%
% \begin{figure}
% 	\centering
% 		\includegraphics[width=0.95\linewidth]{figs/pruning.pdf}
% 	\caption{We propose a stochastic channel pruning algorithm using a Gumbel-softmax trick to generate discrete mask samples from the model with a continuous output space. Our algorithm learns a set of channel selection probability vectors, $\{\textbf{b}_1, ..., \textbf{b}_{N_{pl}}\}$, in each layer, where $\mathbf{b}_l$ indicates which channel is likely to be sampled in the $l^\textrm{th}$ layer. By employing the Gumbel-softmax trick, $\mathbf{b}_l$ generates discrete channel selection mask $M_l$, which is applied to the model parameters $W_l$ to prune the channels.} 
% 	\label{fig:pruning}
% \end{figure} 
% %%%%%%%%%%%%%%%%
% \fi

% \iffalse
% \paragraph{Activation normalization.}
% Due to the imbalance of the size of quantized main network and channel pruned network, channel pruned network is vulnerable to reduce the impact of itself.
% Therefore, similarly to \ref{paragraph:act_norm}, we also apply distribution regularizer for channel pruned activation, which is given by
% \begin{align}
%     \mathcal{L}_\textrm{pA}(A^\textrm{p,bn}) = \sum^{N_l}_{i=1} \begin{pmatrix} \left(\sigma_i - \mathtt{std}(A_i^\textrm{p,bn})\right)_{+}  \\ 
%     +  \left(\mu_i - \mathtt{mean}(A_i^\textrm{p,bn})\right)_{+}\end{pmatrix},
% \end{align}
% where $A^\textrm{p,bn}=\{  A_1^\textrm{p,bn}, ..., A_{N_l}^\textrm{p,bn} \}$ is a set of activations which are the outputs of batch normalization.  
% Finally, total quantization related regularizer loss $\mathcal{L}_\textrm{prune}$ is formulated as below,
% \begin{align}
% 	\mathcal{L}_\textrm{prune} = \mathcal{L}_\textrm{pW} + \mathcal{L}_\textrm{pA}.
% \end{align}
%  \fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \iffalse
% \subsection{Hybrid Representation of Quantiztion and Channel Pruning}
% \ilchae{[Combination of representation and total objective]}

% Our algorithm use combination of representations extracted from quantization network and channel pruned network like 
% \begin{align}
% A_\textrm{comb} = A_\textrm{prune} + A_\textrm{quant}.
% \end{align}
% From combinatorial feature map $A_\textrm{comb}$, each feature of local region proposal $\mathcal{R}_t$ is extracted like $\mathbf{x}_i = \mathtt{RoIAlign}(A_\textrm{comb}; \mathcal{R}_i)$.
% Target score estimation with fully connected layers is totally same with original RT-MDNet.
% For pretraining phase, Similarly to original RT-MDNet, we train our model with multi-domain learning scenario and additional regularizers mentioned in previous section,
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{align}
% \mathcal{L}_\textrm{pre} = \mathcal{L}_{cls} + \mathbf{\lambda}_1 \mathcal{L}_\textrm{inst} + \mathbf{\lambda}_2 \mathcal{L}_\textrm{quant} + \mathbf{\lambda}_3 \mathcal{L}_\textrm{prune} 
% \end{align}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%where $\lambda_1$, $\lambda_2$, $\lambda_3$ are pre-defined coefficients for each component of the objective.
% We learns our learnable parameters by minimizing $\mathcal{L}_\textrm{pre}$. 
% \fi


==> sections/baseline_trackers.tex <==
% !TEX root = ../main.tex
\section{Visual Tracking using Hybrid Representations}
\label{sec:visual}
%The proposed online hybrid representation learning algorithm is applied to visual tracking problem, which requires very efficient online learning at its run-time.
Visual Tracking is one of the  fundamental problem in computer vision and it is good application to test the performance of our algorithm on the streaming data.
The goal of visual tracking is to estimate the location of a target object from sequantially streamed frames of video while the ground-truth bounding box of the target at the first frame is given.
It requires very efficient online learning at its run-time and fine-grained bounding box regression.
%The proposed online hybrid representation learning algorithm is applied to visual tracking problem, which requires very efficient online learning or fine-grained bounding box regression at its run-time.
The overall framework in the context of hybrid representation learning for object tracking is illustrated in Figure~\ref{fig:overall_framework}, where we present two different paths of backpropagation for offline pretraining and online model updates.
In this section, we first describe our baseline trackers, RT-MDNet~\cite{jung2018real} and SiamRPN++~\cite{li2019siamrpn++}, and then discuss how our approach is deployed to accelerate the baseline tracking algorithm.
%%%%%%%%%%%%%%%
\begin{figure*}
	\centering
		\includegraphics[width=0.95\linewidth]{Figures/framework.pdf}
	\caption{Overall framework of our algorithm. We train hybrid representation for both low-bit quantized network ($\mathtt{f}^q$) and light weight full precision network ($\mathtt{f}^p$) on pretraining time while only light weight network is fine-tuned in test phase.
	Red arrow denotes the gradient backpropagation of full precision network in online model update and pretraining while blue arrow denotes the backpropagation in pretraining.}
	\label{fig:overall_framework}
\end{figure*}10 $\sim$ 20$\%$ 
%%%%%%%%%%%%%%%%

\subsection{Background}
\paragraph{RT-MDNet}
The model of RT-MDNet~\cite{jung2018real} has two-stage structure, $\mathtt{f}_\textrm{md}=\{ \mathtt{f}_\textrm{md-conv}, \mathtt{f}_\textrm{md-pred} \}$.
The first stage generates shared feature map from whole image and the second detects target location by observing the shared feature map.
During tracking, the method proceeds online model update.

RT-MDNet conducts pretraining named as multi-domain learning.
A video sequence containing a single independent target is regarded as a single domain. 
From each domain, the target is separated from backgrounds by binary classification, while the target becomes discriminative from the targets of other domain by applying instance embedding learning. 
If $k^\textrm{th}$ domain's image $I$ is given, shared feature map is computed as $A_\textrm{share} = \mathtt{f}_\textrm{md-conv}(I; \mathcal{W}_\textrm{md-conv})$, where $\mathcal{W}_\textrm{md-conv}$ is the set of convolutional model parameters.
After then, current training dataset $\mathcal{D}^k_\textrm{md} = \{ (\mathbf{x}_i, \mathbf{y}_i) \}$ is gathered by including pairs of local region's representation $\mathbf{x}_i$ sampled from the shared feature map and its binary label $\mathbf{y}_i \in \{1,0\}$; 1 denotes the positive while 0 means the negative. 
The domain's classifier  $\mathtt{f}_\mathrm{md-pred}$ computes the binary classification score of each local region, $\tilde{\textbf{y}}^k_i = \mathtt{f}_\textrm{md-pred}(x_i; \mathcal{W}_\textrm{md-pred}, k)  \in \mathbb{R}^2$. 
%The domain's classifier  $\mathtt{f}_\mathrm{md-pred}$ computes the binary classification score of each local region, $\tilde{\textbf{y}}_i = \mathtt{softmax}( \mathtt{f}_\textrm{md-pred}(x_i; \mathcal{W}_\textrm{md-pred}, k))  \in \mathbb{R}^2$ 
%where softmax activation function $\mathtt{softmax}(\cdot)$ normalizes the output into probability-like vector; $\tilde{\textbf{y}}_i[1]$ denotes target score while $\tilde{\textbf{y}}_i[0]$ denotes background score. 
Then, a binary classification loss $\mathcal{L}_\textrm{cls}$ is formularized as
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\label{formula:cross_entropy}
\mathcal{L}_\textrm{cls}(\mathcal{D}^k_\textrm{md}; \mathcal{W}_\textrm{md}) = -\mathbb{E}_{\sim\mathcal{D}^k_\textrm{md}} [\textbf{y}_i \mathtt{log}(\tilde{ \mathbf{y}}^k_i[1] )  + (1-\mathbf{y}_i)\texttt{log}(\tilde{\mathbf{y}}^k_i[0])],
%\mathcal{L}_\textrm{cls}(\mathcal{D}^k_\textrm{md}; \mathcal{W}_\textrm{md}) = -\mathbb{E}_{\sim\mathcal{D}^k_\textrm{md}}\begin{bmatrix} \textbf{y}_i \mathtt{log}(\tilde{ \mathbf{y}}_i[1] ) \\  + (1-\mathbf{y}_i)\texttt{log}(\tilde{\mathbf{y}}_i[0]) \end{bmatrix},
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%
where $\mathcal{W}_\textrm{md}=\{ \mathcal{W}_\textrm{md-conv}, 
\mathcal{W}_\textrm{md-pred} \}$ is the set of all model parameters.
To learn discriminative instance embedding, the instance embedding loss $\mathcal{L}_\textrm{inst}$ is obtained as 
\begin{align}
\mathcal{Y}_i = \mathtt{softmax}([ \tilde{\mathtt{y}}^{0}_{i}[1] , \tilde{\mathtt{y}}^{1}_{i}[1], \dots ,\tilde{\mathtt{y}}^{N_\textrm{inst}}_{i}[1] ]) \in \mathbb{R}^{N_\textrm{inst}}\\
\mathcal{L}_\textrm{inst}(\mathcal{D}^k_\textrm{md}; \mathcal{W}_\textrm{md}) = - \mathbb{E}_{\sim \mathcal{D}^k_\textrm{md}} [\texttt{log}(\mathcal{Y}_{i}[k]) ].
\end{align}

Finally, a total objective of multi-domain learning, denoted as $\mathcal{L}_\textrm{md}$ is formularized as linear combination of the classification loss and instance embedding loss, 
%%%%%%%%%%%%%%
\begin{align}
\mathcal{L}_\textrm{md}(\mathcal{D}_\textrm{md}; \mathcal{W}_\textrm{md}) = 
\mathbb{E}[\mathcal{L}_\textrm{cls}(\mathcal{D}^k_\textrm{md}; \mathcal{W}_\textrm{md}) + \mathbf{\lambda}_\textrm{md} \mathcal{L}_\textrm{inst}(\mathcal{D}^k_\textrm{md}; \mathcal{W}_\textrm{md})] ,
%\mathcal{L}_\textrm{md}(\mathcal{D}_\textrm{md}; \mathcal{W}_\textrm{md}) = 
%\mathbb{E}\begin{bmatrix}\mathcal{L}_\textrm{cls}(\mathcal{D}^k_\textrm{md}; \mathcal{W}_\textrm{md})\\ + \mathbf{\lambda}_\textrm{md} \mathcal{L}_\textrm{inst}(\mathcal{D}^k_\textrm{md}; \mathcal{W}_\textrm{md}) \end{bmatrix},
\end{align}
%%%%%%%%%%%%%%%%
where $\mathcal{D}_\textrm{md}$ is the set of all domain's training set and $\lambda_\textrm{md}$ is the coefficient of balancing two loss functions.

\paragraph{SiamRPN++}
%\ilchae{high-level pipeline of SiamRPN++}
For the second baseline tracker, we employ SiamRPN++~\cite{li2019siamrpn++}.
Its model $\mathtt{f}_\textrm{siam}=\{
\mathtt{f}_\textrm{back}, \mathtt{f}_\textrm{siam-pred}\}$ is based on Siamese networks which formulate the tracking algorithm as a cross-correlation problem between two branches.

Each branch of Siamese networks learns the representation of the target object and the search region, respectively. 
%The first branch of siamese network learns the representation of the target object while the second trains search area. 
Without online model update, the algorithm pretrains the binary object classifier and the bounding-box regressor in a fully offline manner.
Since the support of high-precision is essential for fine-grained bounding box regression, our hybrid representation algorithm allows this tracker to reach the accelerated execution time while maintaining the tracking performance.
%For fine-grained bounding-box regression, it needs the high-precision support and our hybrid representation algorithm can be applied to help this tracker enhance the performance with accelerated execution time.
 

%\ilchae{model detail}
Suppose that a target image $\mathcal{T}$ is given with the initial target state in the first frame of the sequence.
For every frame $\mathcal{U}$, depth-wise cross-correlation $\mathtt{DXCorr}$ is applied to extract similarity-based feature map $A_\textrm{siam}$ between the target $\mathcal{T}$ and the search frame $\mathcal{U}$ as follows:
%%%%%%%%%%%%%%
\begin{align}
A_\textrm{siam}=\mathtt{DXCorr}(\mathtt{f}_\textrm{back}(\mathcal{U}; \mathcal{W}_\textrm{siam-back}), \mathtt{f}_\textrm{back}(\mathcal{T}; \mathcal{W}_\textrm{siam-back})),
\end{align}
%%%%%%%%%%%%%%%
where $\mathtt{f}_\textrm{back}$ and $\mathcal{W}_\textrm{siam-back}$ are backbone network and the set of backbone network's parameters, respectively.
Then, a classification score map $S_\textrm{cls} \in \mathbb{R}^{H \times W \times (N_A \times 2) }$ and a bounding box regression map $S_\textrm{loc} \in \mathbb{R}^{H \times W \times (N_A \times 4)} $ is computed by observing $A_\textrm{siam}$ via prediction network $\mathtt{f}_\textrm{siam-pred}$,
%%%%%%%%%%%%%%%%%
\begin{align}
S_\textrm{cls}, S_\textrm{loc} = \mathtt{f}_\textrm{siam-pred}(A_\textrm{siam}; \mathcal{W}_\textrm{siam-pred}),
%S_\textrm{cls}=\mathtt{f}_\textrm{cls}(A_\textrm{siam}; \mathcal{W}_\textrm{siam}) \in \mathbb{R}^{H \times W \times (N_A \times 2) }\\ 
%S_\textrm{loc}=\mathtt{f}_\textrm{loc}(A_\textrm{siam}; \mathcal{W}_\textrm{siam}) \in \mathbb{R}^{H \times W \times (N_A \times 4)},
\end{align}
where $N_A$ is the number of anchors and $\mathcal{W}_\textrm{siam-pred}$ is the set of prediction network's parameters, respectively.
A single vector of $S_\textrm{cls}$ predicts binary classification scores discriminating target position from background while a single vector of $S_\textrm{loc}$ predicts the differences between current anchor and ground-truth of bounding box.
%The detailed structure of bounding box regressor output is same as SiamRPN~\cite{li2018high} and the response maps are aggregated from different layers as from backbone networks.
%For the sake of convenience, we will call the combined response maps as $S_\textrm{cls}$ and $S_\textrm{loc}$. 
Finally, the region with maximum classification score is selected and the final bounding box is aligned by observing the output of the regressor.

%\ilchae{Training loss}
For pretraining phase, SiamRPN++ samples training dataset $\mathcal{D}_\textrm{siam}=\{ (\mathcal{U}_i, \mathcal{T}_i)  \}$ by applying the same protocol as \cite{li2018high}.  
Then, it minimizes the loss function $\mathcal{L}_\textrm{siam}$ including a binary classification loss  $\mathcal{L}_\textrm{cls}$ and a bounding box regression loss $\mathcal{L}_\textrm{loc}$,
\begin{align}
\mathcal{L}_\textrm{siam}(\mathcal{D}_\textrm{siam}; \mathcal{W}_\textrm{siam}) = \mathcal{L}_\textrm{cls}(S_\textrm{cls}; \mathcal{W}_\textrm{siam}) \nonumber 
+ \lambda_\textrm{siam} \mathcal{L}_\textrm{loc}(S_\textrm{loc}; \mathcal{W}_\textrm{siam}),
\end{align} 
where $\mathcal{W}_\textrm{siam}=\{\mathcal{W}_\textrm{siam-back}, \mathcal{W}_\textrm{siam-pred}\}$ is the set of model parameters  and $\lambda_\textrm{siam}$ is the coefficient.
More details of the loss function are introduced in ~\cite{li2018high}.

\subsection{Training for Quantized and Pruned Network}
%\ilchae{[New loss function for mdnet]}
For the application of hybrid representation in RT-MDNet, we prepare the set of hybrid model parameters $\mathcal{W}^{h}_\textrm{md} = \{  \mathcal{W}^{q}_\textrm{md-conv},\mathcal{W}^{p}_\textrm{md-pred}, \mathcal{W}^{p}_\textrm{md-cls} \}$, where the parameters $\mathcal{W}^p_{*}$ and $\mathcal{W}^q_{*}$  mean the pruned model's parameters and and quantization model's parameters transferred from the original parameters $\mathcal{W}_{*}$, respectively. 
From given $k^\textrm{th}$ domain's image $I$, We extract hybrid shared feature map $A^h_\textrm{share}$ by employing parallel primary and residual networks as follows:
\begin{align}
A^h_\textrm{share} = \mathtt{f}^q_\textrm{md-conv}(I, \mathcal{W}^q_\textrm{md-conv}) + \mathtt{f}^p_\textrm{md-conv}(I, \mathcal{W}^p_\textrm{md-conv}),
\end{align} 
where $\mathtt{f}^q_\textrm{md-conv}$ and $\mathtt{f}^p_\textrm{md-conv}$ are quantization application of and pruning application of $\mathtt{f}_\textrm{md-conv}$, respectively.
We sample
$k^\textrm{th}$ domain's training dataset $\mathcal{D}^k_\textrm{md} = \{ (\mathbf{x}_i, \mathbf{y}_i) \}$ by observing $A^h_\textrm{share}$.
To compute prediction score $\tilde{y}^k_i$, we apply channel pruned classifier $\mathtt{f}^p_\textrm{cls}$ only:
\begin{align}
	\tilde{y}^k_i = \mathtt{f}^p_\textrm{md-pred} (\mathbf{x}_i; \mathcal{W}^p_\textrm{md-pred},k).
\end{align}
We construct the objective loss $\mathcal{L}_\textrm{md-total}$, the combination of original RT-MDNet's loss and our hybrid training loss as, 
\begin{align}
\mathcal{L}_\textrm{md-total} = \mathcal{L}_\textrm{cls}(\mathcal{D}^k_\textrm{md}; \mathcal{W}^h_\textrm{md}) + \lambda_\textrm{md}\mathcal{L}_\textrm{inst}(\mathcal{D}^k_\textrm{md}; \mathcal{W}^h_\textrm{md}) + \mathbf{\lambda}_1 \mathcal{L}_\textrm{quant} + \mathbf{\lambda}_2 \mathcal{L}_\textrm{prune},
\end{align}

where $\lambda_1$, $\lambda_2$ are pre-defined coefficients for each component of the objective.
We learn our learnable parameters by minimizing $\mathcal{L}_\textrm{md-total}$. 

%\ilchae{[New loss function for SiamRPN++]}
For hybrid representation learning for SiamRPN++, we prepare the set of hybrid model parameters $\mathcal{W}^h_\textrm{siam}=\{ \mathcal{W}^q_\textrm{siam}, \mathcal{W}^p_\textrm{siam}   \}$.
Similarly to SiamRPN++, parallel primary and residual networks compute hybrid representation map and correlated depth-wise similarity maps $A_\mathcal{U}^h$ and $A_\mathcal{T}^h$ as follows:
\begin{align}
	&A_{\star}^h = \mathtt{f}^p_\textrm{back}({\star}; \mathcal{W}^p_\textrm{siam-back}) + \mathtt{f}^q_\textrm{back}({\star}; \mathcal{W}^q_\textrm{siam-back}), \nonumber \\
     	%A_\mathcal{U}^h = \mathtt{f}^p_\textrm{back}(\mathcal{U}; \mathcal{W}^p_\textrm{siam}) + \mathtt{f}^q_\textrm{back}(\mathcal{U}; \mathcal{W}^q_\textrm{siam})\\
	%A_\mathcal{T}^h = \mathtt{f}^p_\textrm{back}(\mathcal{T}; \mathcal{W}^p_\textrm{siam}) + \mathtt{f}^q_\textrm{back}(\mathcal{T}; \mathcal{W}^q_\textrm{siam})\\
	&A^h_\textrm{siam} = \mathtt{DXCorr}(A_\mathcal{U}^h, A_\mathcal{T}^h ),
\end{align}
where $\star \in \{ \mathcal{U}, \mathcal{T} \}$. Then, hybrid representation is constructed at classification and bounding-box regression score,
$S^h_\textrm{cls}, S^h_\textrm{loc} = \mathtt{f}^h_\textrm{siam}(A^h_\textrm{siam}; \mathcal{W}^h_\textrm{siam})$. 
And then, the total objective of hybrid SiamRPN++ is obtained by
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathcal{L}_\textrm{siam-total} = \mathcal{L}_\textrm{cls}(S^h_\textrm{cls};\mathcal{W}^h_\textrm{siam}) + \lambda_\textrm{siam}\mathcal{L}_\textrm{loc}(S^h_\textrm{loc};\mathcal{W}^h_\textrm{siam} ) +  \mathbf{\lambda}_1 \mathcal{L}_\textrm{quant} + \mathbf{\lambda}_2 \mathcal{L}_\textrm{prune} . %+ \mathcal{L}_\textrm{track}. 
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\ilchae{[training strategy (pretrain and online)]}
Our framework trains both parameters of quantized network $\mathcal{W}^q_{*}$ and channel-pruned network $\mathcal{W}^p_{*}$ in pretraining time. 
On the other hand, from online model update in the test time, we freeze the parameters of quantized network to maintain time-invariant information while the lightweight full precision network update its parameters for adaptation to time-variant information.

\iffalse
\ilchae{[new loss function ]}
Similarly to RT-MDNet, we adopt multi-domain learning strategy in pretraining phase.
$k^\textrm{th}$ domain's training dataset $\mathcal{D}^k = \{ (\mathbf{x}_i, \mathbf{y}_i) \}$ includes pairs of local region's representation $\mathbf{x}_i$ and its binary label $\mathbf{y}_i \in \{1,0\}$; 1 denotes the positive label while 0 means the negative label. 
Shared feature map is generated by employing our hybrid representation.
The domain's classifier  $\mathtt{f}^{k}_\mathrm{cls}$ computes the binary classification score of each local region, $\tilde{\textbf{y}}_i = \mathtt{softmax}( \mathtt{f}^k_\textrm{cls}(x_i))  \in \mathbb{R}^2$ 
where softmax activation function $\mathtt{softmax}(\cdot)$ normalizes the output into probability-like vector; $\tilde{\textbf{y}}_i[1]$ denotes target score while $\tilde{\textbf{y}}_i[0]$ denotes background score. 
Then, binary classification loss $\mathcal{L}_\textrm{cls}$ is formularized as
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\label{formula:cross_entropy}
\mathcal{L}_\textrm{cls}(\mathcal{D}^k; \mathcal{W}^p, \mathcal{W}^q) = - \mathbb{E}_{(\mathbf{x}_i, \mathbf{y}_i) \sim \mathcal{D}^k}[\textbf{y}_i \mathtt{log}(\tilde{ \mathbf{y}}_i[1] ) \nonumber \\ + (1-\mathbf{y}_i)\texttt{log}(\tilde{\mathbf{y}}_i[0])].
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%
To learn discriminative instance embedding, we firstly compute output score, denoted as $\mathcal{Y}_i$ which concatenates target positive scores of  $\mathbf{x}_i$ from $N_\textrm{inst}$ domains
%%%%%%%
\begin{align}
\mathcal{Y}_i = \mathtt{softmax}([\mathtt{f}^1_{\textrm{cls}}(\mathbf{x}_{i})[1]  , \mathtt{f}^2_{\textrm{cls}}(\mathbf{x}_{i} )[1], \dots ,\mathtt{f}^{N_\textrm{inst}}_{\textrm{cls}}(\mathbf{x}^k_{i}; W^{N_\textrm{inst}}_\mathrm{fc})[1]]) \in \mathbb{R}^{N_\textrm{inst}},
\end{align}
%%%%%%%
Then, the instance embedding loss $\mathcal{L}_\textrm{inst}$ is obtained as 
%%%%%%%
\begin{align}
\mathcal{L}_\textrm{inst}(\mathcal{D}^k; \mathcal{W}^p, \mathcal{W}^q ) = - \mathbb{E}_{x_i \sim \mathcal{D}^k} [\texttt{log}(\mathcal{Y}_{i}[k]) ],
\end{align}
%\begin{align}
%\mathcal{L}_\textrm{inst}(\mathcal{D}^k; \mathcal{W}^p, \mathcal{W}^q ) = - \mathbb{E}_{x_i \sim \mathcal{D}^k} [\texttt{log}(\mathcal{Y}_{i}[k]) + \sum_{j \neq k}{\texttt{log}(1-\mathcal{Y}_i[j])}],
%\end{align}
%%%%%%%
Total objective of multi-domain learning, denoted as $\mathcal{L}_\textrm{md}$ is formularized as linear combination of the classification loss and instance embedding loss, 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathcal{L}_\textrm{md}(\mathcal{D}; \mathcal{W}^p, \mathcal{W}^q) = 
\mathbb{E}_{ \mathcal{D}^k \sim \mathcal{D} } [ \mathcal{L}_{cls}(\mathcal{D}^k; \mathcal{W}^p, \mathcal{W}^q) + \mathbf{\lambda}_1 \mathcal{L}_\textrm{inst}(\mathcal{D}^k; \mathcal{W}^p, \mathcal{W}^q) ],
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\mathcal{D}$ is the set of all domain's training set and $\lambda_1$ is coefficient for instance embedding loss..
Finally, the total objective of pretraining is obtained by
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathcal{L}_\textrm{pre} = \mathcal{L}_{cls} + \mathbf{\lambda}_1 \mathcal{L}_\textrm{inst} + \mathbf{\lambda}_2 \mathcal{L}_\textrm{quant} + \mathbf{\lambda}_3 \mathcal{L}_\textrm{prune} 
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\lambda_2$, $\lambda_3$ are pre-defined coefficients for each component of the objective.
	We learn our learnable parameters by minimizing $\mathcal{L}_\textrm{pre}$. 


%\ilchae{[training strategy (pretrain and online)]}
Our framework trains both parameters of quantized network $\mathcal{W}^q$ and channel-pruned network $\mathcal{W}^p$ in pretraining time. 
On the other hand, from online model update in the test time, we freeze the parameters of quantized network to maintain time-invariant information while the lightweight full precision network adapt update its parameters for adaptation to time-variant information.
We employ same online model update strategy with RT-MDNet.
\fi

\iffalse
\subsection{Model Structure}
\ilchae{[explanation of data flow in model structure]}
We employ RT-MDNet~\cite{jung2018real} as our baseline tracker.
\ilchae{RT-MDNet consists of two-stage framework including convlution network and fully-connected network $\texttt{f}_\textrm{fc}$.
Convolution network computes feature map extracted from whole input image. 
From our application, we employ our hybrid networks, quantized network and light-weight network as the convolution network.
}
\iffalse
RT-MDNet consists of two-stage framework including convolution network $\texttt{f}_\textrm{conv}$ and fully-connected network $\texttt{f}_\textrm{fc}$. 
Convolution network computes feature map $A_\textrm{conv}$ extracted from whole input image $A_{0}$ 
The feature map is generated by forward passing input image to sequential $N_l$ convolutional layers 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\label{formula:conv_layer}
    %\begin{matrix}
        A_{i} = \sigma(A_{i-1} * W_{i} ) \text{ for } i=1...N_l \\
        A_\textrm{conv} = \texttt{f}_\textrm{conv} (A_{0}; W_\textrm{conv}) = A_{N_l}, 
    %\end{matrix}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\sigma$ is non-linear activation functions including ReLU and local response normalization (LRN) coming after convolution operation $*$.
It defines set of convolution layer's parameters as $W_\textrm{conv}=\{W_i\}_{i=1,,,N_l}$ where its convolution network consists of three convolution layers ($N_l = 3$).
\fi

By employing a $\texttt{RoIAlign}$ layer introduced in ~\cite{he2017mask}, each representation $\mathbf{x}_i =\texttt{RoIAlign}(A_\textrm{hyb},\mathcal{R}_i)$ allocated to the local region proposal $\mathcal{R}_i$ is sampled from the shared feature map $A_\textrm{conv}$.
Then, fully-connected network estimates its target score $\tilde{\mathbf{y}}_{i} = \mathtt{softmax}( \texttt{f}_\textrm{fc} (\mathbf{x}_i; W_\textrm{fc})) \in \mathbb{R}^{2}$ indicating whether the candidate is on the target or background.
Its fully-connected network includes three basic fully connected layers ($\texttt{fc}4 - 6$).


\ilchae{common objective (classification loss) in train and test time]}
To learn binary classification discriminate between target object and backgrounds, it employs binary cross entropy objective 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\label{formula:cross_entropy}
    \mathcal{L}_\textrm{cls}(\mathcal{D}; W^p, W^q, W_\textrm{fc}) = - \mathbb{E}_{(\mathbf{x}_i, \mathbf{y}_i) \sim \mathcal{D}}[\textbf{y}_i \mathtt{log}(\tilde{ \mathbf{y}}_i[1] )  + (1-\mathbf{y}_i)\texttt{log}(\tilde{\mathbf{y}}_i[0])],
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where training dataset $\mathcal{D}=\{(\mathbf{x}_i, \mathbf{y}_i, \mathcal{R}_i)\}$ includes tuples of local region $\mathcal{R}_i$ and its representation $\mathbf{x}_i$ sampled after $\texttt{RoIAlign}$ layer and its binary label $\mathbf{y}_i \in \{1,0\}$; 1 denotes the positive label while 0 means the negative label.

\subsubsection{Pre-Training: Multi-Domain Learning}
\ilchae{[Multi domain initialization]}
Similarly to pretraining in MDNet, multi-domain learning is applied for the purpose of adaptation to class-agnostic targets in the object tracking task.
From multi-domain learning, a video sequence containing a single independent target is regarded as a single separated domain and binary classification between the target and backgrounds is independently learned for each domain.  
Each binary classifier allocated to a $k^\textrm{th}$ domain trains separated branch of $\texttt{fc}^{k}_{6}$ layer while the fore-head of network ($\mathtt{Conv1-3}$, $\texttt{fc}4-5$) is shared for every domain.  
Parameters of $k^\textrm{th}$ domain's fully-connected network are defined as $W^{k}_\textrm{fc}=\{ W_{\textrm{fc}_4}, W_{\textrm{fc}_5}, W_{\textrm{fc}^k_6}\}$ in pretraining phase.
Note that the separated branches of $\texttt{fc}^{k}_{6}$ layers in the pretraining phase are discarded and a single randomly initialized $\texttt{fc}_6$ layer is used for the test phase. 

\ilchae{[Multi-domain learning objective]}
From each single domain $k$, the objective function consists of a classification loss $\mathcal{L}_\textrm{cls}$ and an instance embedding loss $\mathcal{L}_\textrm{inst}$. 
The instance embedding loss is designed to make each domain's target object distant from the instances of other domains.
It concatenates target positive scores of $k^\textrm{th}$ domain's target instance sample $\mathbf{x}^k_i$ from all $N_\textrm{inst}$ domain  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathcal{Y}_i = \mathtt{softmax}([\mathtt{f}_{\textrm{fc}}(\mathbf{x}^k_{i}; W^1_\mathrm{fc})[1], \mathtt{f}_{\textrm{fc}}(\mathbf{x}^k_{i}; W^2_\mathrm{fc})[1],,,\mathtt{f}_{\textrm{fc}}(\mathbf{x}^k_{i}; W^{N_\textrm{inst}}_\mathrm{fc})[1]]) \in \mathbb{R}^{N_\textrm{inst}}.
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Then, the instance embedding loss is formularized as below
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathcal{L}_\textrm{inst}(\mathcal{D}^\textrm{k}; W^p, W^q, \{ W^t_\textrm{fc} \}_{t=1,,,N_\textrm{inst}}) = - \mathbb{E}_{x_i \sim \mathcal{D}^k} [\texttt{log}(\mathcal{Y}_{i}[k]) + \sum_{j \neq k}{\texttt{log}(1-\mathcal{Y}_i[j])}],
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\mathcal{D}^k$ is the sub-dataset sampled from  $k^\textrm{th}$ domain.
It discriminates sample instance of $k^\textrm{th}$ domain from other. 
Finally, total pretraining objective $\mathcal{L}_\textrm{pre}$ is formularized as linear combination of the classification loss and instance embedding loss, 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathcal{L}_\textrm{pre}(\mathcal{D}; W) = \mathbb{E}_{k \sim \texttt{uniform}() } [ \mathcal{L}_{cls}(\mathcal{D}^k; W) + \mathbf{\lambda} \mathcal{L}_\textrm{inst}(\mathcal{D}^k; W) ],
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $W$ contains all model parameters and $\texttt{uniform}()$ draw index of domain from in uniform distribution.

\ilchae{
For pretraining phase, Similarly to original RT-MDNet, we train our model with multi-domain learning scenario and additional regularizers mentioned in previous section,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathcal{L}_\textrm{pre} = \mathcal{L}_{cls} + \mathbf{\lambda}_1 \mathcal{L}_\textrm{inst} + \mathbf{\lambda}_2 \mathcal{L}_\textrm{quant} + \mathbf{\lambda}_3 \mathcal{L}_\textrm{prune} 
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%where $\lambda_1$, $\lambda_2$, $\lambda_3$ are pre-defined coefficients for each component of the objective.
We learn our learnable parameters by minimizing $\mathcal{L}_\textrm{pre}$. 
}


\subsection{Online Tracking Strategy}
Due to target-specific adaptation in test time, RT-MDNet adjust online model update with accumulated dataset online according to the update strategy in \cite{nam2016learning}. 
\ilchae{Write later or not.} 

%%%%%%%%%%%%%%%
\begin{figure}
	\centering
%	\includegraphics[width=0.99\linewidth]{Figures/overall_framework.png}
	\caption{\ilchae{Overall framework of our algorithm. We train hybrid representation for both low-bit quantized network and light-weight full precision network on pretraining time while only light-weight network is fine-tuned in online update.
	Red arrow denotes the gradient backpropagation in online model update while blue arrow deotes the backpropagation in pretraining.} }
	\label{fig:weight_dist}
\end{figure}
%%%%%%%%%%%%%%%%
\fi






==> sections/discussions.tex <==
% !TEX root = ../hybrid_tracking.tex

%\clearpage
\section*{Discussions}
\label{sec:discussions}
Our work is about learning hybrid lightweight representations with low-bit quantization and channel pruning strategy.
Light-scale deep neural networks can be applied to industrial projects dealt with streaming data effectively.
In the real world situation, streaming data often can be analyzed in real-time and  be driven on device-system.
From autonomous driving system to researches in military purpose, Attaching lightweight module is inevitably applied.  
However, technologies in military service can be critical to the peace of world.
Fortunately, object tracking is also applicable to robust defence system.
In the view of the limitation of our method, quantization methods is not stand-alone algorithm, but the support of hardware optimization is needed to maximize its performance. 

==> sections/methods_bak.tex <==
% !TEX root = ../main.tex
\section{Online Representation Learning using Quantized and Pruned Networks}
\label{sec:online}
This section describes the architecture of our deep neural network and the offline and online training strategies for robust feature representations.

\subsection{Overview}
\label{sub:overview}
Our main idea is to represent an image using an ensemble of two lightweight deep neural networks, where one is a quantized network based on a low bit-width and the other is compressed by a channel pruning algorithm.
The former network plays a role as a backbone network while the latter encodes time-varying residual information.
The proposed algorithm is composed of two parallel networks for learning accurate representations, but updates the residual network only for online learning to minimize run-time complexity.
%Contrary to the prior studies~\cite{jung2019learning, gong2019differentiable}, which adopt fully connected layers in full precision on top of quantized convolutional layers for stable online learning, 


\iffalse
This section presents our light-weightening algorithm including combination of low-bit quantization and model channel pruning.
We light-weighten convolutional network while fully-connected network maintains full precision and full channels. 
Different from previous quantization studies on image classification task~\cite{jung2019learning, gong2019differentiable}, fully-connected network should maintain full precision for the stability of online model update and bounding box regression in test phase.
Our algorithm adds two representations from low-bit quantization network and channel pruned network to complement the information loss from the sparsity of low-bit representation. 
\fi


Let $\mathtt{f}_\mathrm{conv}(\cdot ; \cdot)$ be a standard convolutional neural network parametrized by a set of parameters in $N_l$ convolutional layers, $\mathcal{W}_\textrm{conv} = \{ W_l \}_{l=1:N_l}$.
Then, the final output feature map $A_\textrm{conv}$ is given by feedforwarding an input image $A_0$ to the $N_l$ layers as follows:
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\label{formula:conv_layer}
%\begin{matrix}
A_{i} & = \sigma(A_{i-1} * W_{i} ), ~~~ \text{ for } i=1...N_l, \\
A_\textrm{conv} & = A_{N_l} = \texttt{f}_\textrm{conv} (A_{0}; \mathcal{W}_\textrm{conv}), 
%\end{matrix}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\sigma(\cdot)$ denotes a non-linear activation function and $*$ indicates the convolution operator.
Contrary to the standard conventional neural networks, our framework learns two parallel networks---one is a quantized network $\mathtt{f}_\textrm{quant} $ and the other is a channel-pruned network $\mathtt{f}_\textrm{prune}$.
Denote by $\mathcal{W}^q = \{ W^q_l \}_{l=1:N_l}$ and $\mathcal{W}^p = \{ W^p_l \}_{l=1:N_l}$ the $N_b$-bit quantized parameters of the backbone network and the channel-pruned parameters in the residual branch, respectively.
Then, the proposed hybrid representation, $A_\textrm{hybrid}$, is computed by the summation of the feature maps from the quantized and pruned networks as follows:
%%%%%%%%
\begin{align}
A_\textrm{hybrid} & = A_\textrm{quant} + A_\textrm{prune} \nonumber \\
& = \mathtt{f}_\textrm{quant}(A_0; \mathcal{W}^q) + \mathtt{f}_\textrm{prune}(A_0; \mathcal{W}^p),
\end{align}
%%%%%%%%
where $A_\textrm{quant} = \mathtt{f}_\textrm{quant}(A_0; \mathcal{W}^q)$ and $A_\textrm{prune} = \mathtt{f}_\textrm{prune}(A_0; \mathcal{W}^p)$.


\subsection{Low-Bit Quantization of Primary Network}
\label{sub:low-bit}
We quantize both network parameters, $\mathcal{W}_\textrm{conv} = \{W_{l}\}_{l=1:N_l}$, and feature activations, $\mathcal{A} = \{A_l \}_{l=1:N_l}$, in convolutional networks based on \cite{jung2019learning}.
Similarly to \cite{jung2019learning}, our algorithm applies the following low-bit quantization technique to all layers except the input image of the first convolution layer and the output of the last convolution layer.  

\paragraph{Parameter quantization}
Similarly to the output activation, the original model parameters $w_l \in W_l$ are transformed to $\hat{w} \in \hat{W}_l$, which is in the range of $[-1, 1]$, by learning $(c^l_W, d^l_W, \gamma_W^l)$ and computing the following equation:
%
\begin{equation}
    \hat{w}_{l} =
        \begin{cases}
            \texttt{sign}(w_{l}) & \text{if $|w_{l}| > c^l_{W} + d^l_{W}$ } \\
            0 & \text{if $|w_{l}| < c^l_{W} - d^l_{W}$ } \\
            \texttt{sign}(w_{l}) \cdot (\alpha^l_{W} |w_{l}| + \beta^l_{W})^{\gamma^l_{W}} & \text{otherwise},
        \end{cases}
\label{eq:quantization_w}
\end{equation}
%
where $\alpha^l_{W} = 0.5/d^l_{W}$ and $\beta^l_{W}= -0.5 c^l_{W} / d^l_{W} + 0.5$.
The final quantized parameter, $W^q_l$  is obtained by applying the rounding function to the individual elements in $\hat{W}$, which is given by
%
\begin{equation}
W^q_l =  \frac{\texttt{round}(\hat{W}_l \cdot (2^{N_b-1}-1))}{2^{N_b-1}-1}.
\label{eq:quantize_w}
\end{equation}
%


%\ilchae{[Explanation of acitivation quantization]}
\paragraph{Activation quantization}
We convert all the activations in each convolutional layer within the range $[0, 1]$ by a clipped linear transformation.
Let $A_l$ be the output activation of the $l^\textrm{th}$ convolutional layer and $a_l$ be its single element.
Then, the transformation is given by learning the center and the width of the activation interval, denoted by $c^l_{A}$  and $d^l_{A}$, respectively, and applying the following equation:
%
\begin{equation}
    \hat{a}_l \equiv \mathtt{trans}_A^l(a_l) = 
            \begin{cases}
            1 & \text{if $a_l > c^l_{A} + d^l_{A}$ } \\
            0 & \text{if $a_l < c^l_{A} - d^l_{A}$ } \\
            \alpha^{l}_{A} A_l + \beta^{l}_{A} & \text{otherwise},
        \end{cases}
\label{eq:quantization_a}
\end{equation}
%
where $\alpha^l_{A} = 0.5/d^l_{A}$ and $\beta^l_{A}= -0.5 c^l_{A} / d^l_{A} + 0.5$.
In other words, $[c^l_{A} - d^l_{A}, c^l_{A} + d^l_{A}]$ is transformed linearly to $[0, 1]$.
The final quantization output, $A^q_l$ is given by applying the a rounding function, $\mathtt{round}(\cdot)$ to the individual elements in $\hat{A}_l$ as
%
\begin{equation}
A^q_l = \mathtt{quantize}(\hat{A_l}) = \frac{\texttt{round}(\hat{A}_l \cdot (2^{N_b}-1))}{2^{N_b}-1},
\label{eq:quantize}
\end{equation}
%
where $N_b$ is the bit capacity and $\mathtt{quantize}(\cdot)$ denotes the quantization function.
%We define whole matrix-wise transformation as $\mathtt{trans}^l_A() \textrm{ s.t. }  \hat{A}_l=\mathtt{trans}^l_A(A_l)$.


The activation in each layer of a quantized network is given by 
\begin{align}
A^q_{l+1} &= \mathtt{quantize} ( \mathtt{trans}^l_A( \sigma (A^q_l * W^q_{l+1}) ) ), & l &= 0 \dots N_{l}-2 \\
A^q_{N_l} &= \sigma (A^q_{N_l-1} * W^q_{N_l}), & l &= N_l - 1,
\end{align}
%
where $\mathtt{quantize}(\cdot)$ and $\mathtt{trans}^l_A(\cdot)$ are defined in \eqref{eq:quantization_a} and \eqref{eq:quantize}, respectively, and $*$ denote the convolution operator.
The representation of the final convolutional layer, denoted by $A_\textrm{quant}$, is obtained by applying the quantization network, $\texttt{f}_\textrm{quant}$, as follows:
%
\begin{equation}
A_\textrm{quant}=\texttt{f}_\textrm{quant}(A_0; \mathcal{W}^q),
\end{equation}
where $ \mathcal{W}^q =  \{ W^q_l  \}_{l=1,,,N_l} $ is a set of quantized model parameters.


%\ilchae{[weight normalization with standard distribution]}
\paragraph{Weight normalization}
Clipping model parameters located outside the interval $[c_W^l - d_W^l, c_W^l + d_W^l]$ leads to losing details in the quantized representations and make training substantially more difficult.
It turns out that the final accuracy is sensitive to the initialization of $(c^l_W, d^l_W, \gamma_W^l)$, which is aggravated when the quantization is based on lower bits\footnote{When we attempted the network quantization based on \cite{jung2019learning}, 5-bit quantization was much easier than 4-bit counterpart.}.
To alleviate the limitation, we propose a simple but effective regularizer to make a majority of parameters located within the interval, which is given by
%
\begin{align}
    \mathcal{L}_\textrm{quant}(W_\textrm{conv}) = \sum^{N_l}_{i=1}  (\mathtt{mean}({ |\hat{W}_{i}|^{\frac{1}{\gamma^l_W}}  }) - 0.5)^2   + (\mathtt{std}({  | \hat{W}_{i}|^{\frac{1}{\gamma^l_W}} })-0.25)^2 ,
\end{align}
%
where $\mathtt{mean}(\cdot)$ and $\mathtt{std}(\cdot)$ denote mean and standard deviation of all entries in their input matrices, respectively, $| \cdot |$ returns an absolute value matrix of the same size of its input.
By enforcing the distribution of model parameters using this regularizer, we can find more appropriate parameters ($c^l_W, d^l_W, r^l_W$) and train the network faster.
%Although it enforced the specific distribution of model parameters, adjustment with exponential operation of $\gamma$ enables the variety of parameter distributions. 


\iffalse
Therefore, initializing proper value for interval-related parameters is very important and the accuracy is sensitive to the initialization.
To recover the problem, we propose the additional but simple regularizer to let more parameters locate at inner interval.
Based on the meaning of mean and standard deviation in statistics, we regularize the distribution of elements in $\hat{W}_l$ that all elements are in range of $(0,1)$ like
%
where $\mathtt{Std}(*)$ and $\mathtt{Avg}(*)$ returns standard deviation of and average of $*$, respectively.
This regularizer force almost all model parameters to locate at inner range of the interval and makes learning more efficient.
\fi



\subsection{Channel Pruning of Residual Network}
\label{sub:channel}

%\ilchae{[Explanation of gumbel softmax application to model channel pruning]}
We propose a stochastic channel pruning algorithm using a Gumbel-softmax trick to generate discrete samples from the model with a continuous output space.
Our algorithm learns a set of channel selection probability vectors, $\{ \mathbf{b}_l \}_{l=1:(N_l-1)}$, in each layer, where $\mathbf{b}_l$ indicates which channel is likely to be sampled in the $l^\textrm{th}$ layer.
By employing the Gumbel-softmax trick introduced in \cite{jang2016categorical}, $\mathbf{b}_l$ generates discrete channel selection mask $M_{l}$, which is given by
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\label{formula:pruning}
    %\begin{matrix}
\bar{M}_l[i] & = \frac{\texttt{exp}\left( (g_i + \texttt{log} (\mathbf{b}_l[i])/\tau \right) }{ \texttt{exp} \left( (g_i + \texttt{log} (\mathbf{b}_l[i])/\tau \right) + \texttt{exp} \left( (g_i + \texttt{log}(1- \mathbf{b}_l[i]))/\tau \right) } \\
M[i] & = \texttt{round}(\bar{M}[i]) 
    %\end{matrix}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $g_i$ represents a random noise sample from Gumbel distribution $\mathtt{Gumbel}(0,1)$ and $\tau$ is a hyperparameter for temperature.
Similarly to \cite{jang2016categorical}, we apply the straight-through Gumbel estimator for gradient approximation in backpropagation.
In the forward pass of training, we apply the pruning mask $M_{l}$ to the output activation  $A^p_l$ in the $l^\textrm{th}$ layer as
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
    A^p_{l} &= \sigma ( A^p_{l-1} * W^p_{l} ) \odot M_{l},
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $l =1 \dots N_l-1$ and $\odot$ denotes an element-wise multiplication.
Note that a channel whose channel selection probability is below the threshold is removed during testing.
The representation of the final convolution layer, denoted by $\mathtt{f}_\textrm{prune}$, is obtained by applying the pruned network $\mathtt{f}_\textrm{prune}(\cdot ; \cdot)$, as follows:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
A_\textrm{prune} =  \mathtt{f}_\textrm{prune}(A_0; \mathcal{W}^p),
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $ \mathcal{W}^p = \{ W^p_l \}_{l=1,,,N_l}$ is the set of pruned convolution layer's parameters.

%\ilchae{[Explanation of objective for channel pruning]}
For training, channel selecting probabilities $ \{ \mathbf{b}_l \}^{N_l}_{l=2}$ are learned by minimizing the following loss term $\mathcal{L}_\textrm{prune}$ to penalize the number of active channels,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
    \mathcal{L}_\textrm{prune} = \sum^{N_l}_{l=2} \mathbb{E}_{\mathtt{Gumbel}(0,1)}  [  \mathtt{mean}(M_{l}) ].
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
\subsection{Hybrid Representation of Quantiztion and Channel Pruning}
\ilchae{[Combination of representation and total objective]}

Our algorithm use combination of representations extracted from quantization network and channel pruned network like 
\begin{align}
A_\textrm{comb} = A_\textrm{prune} + A_\textrm{quant}.
\end{align}
From combinatorial feature map $A_\textrm{comb}$, each feature of local region proposal $\mathcal{R}_t$ is extracted like $\mathbf{x}_i = \texttt{RoIAlign}(A_\textrm{comb}; \mathcal{R}_i)$.
Target score estimation with fully connected layers is totally same with original RT-MDNet.
For pre-training phase, Similarly to original RT-MDNet, we train our model with multi-domain learning scenario and additional regularizers mentioned in previous section,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathcal{L}_\textrm{pre} = \mathcal{L}_{cls} + \mathbf{\lambda}_1 \mathcal{L}_\textrm{inst} + \mathbf{\lambda}_2 \mathcal{L}_\textrm{quant} + \mathbf{\lambda}_3 \mathcal{L}_\textrm{prune} 
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%where $\lambda_1$, $\lambda_2$, $\lambda_3$ are pre-defined coefficients for each component of the objective.
We learns our learnable parameters by minimizing $\mathcal{L}_\textrm{pre}$. 
\fi


==> sections/methods_old.tex <==
% !TEX root = ../main.tex
\section{Online Hybrid Representation Learning}
%\section{Online Representation Learning using Quantized and Pruned Networks}
\label{sec:online}
%This section describes the proposed deep neural network architecture with the offline and online training strategies for robust hybrid feature representations.

\subsection{Overview of Hybrid Representation}
%\subsection{Overview}
\label{sub:overview}
% Our main idea is to enhance the expressiveness of the convolutional feature extractor by exploiting an ensemble of two lightweight deep neural networks, a quantized network (Section~\ref{sub:low-bit}) and a channel-pruned network (Section~\ref{sub:channel}). 
Our main idea is to enhance the quality of representation of the convolutional feature extractor by exploiting an ensemble of two lightweight deep neural networks, a quantized network (Section~\ref{sub:low-bit}) and a channel-pruned network (Section~\ref{sub:channel}).  
%The quantization network is responsible for feature encoding of primary information while the channel-pruned model enhances the learned representations with high-precision residual information. 
The quantized network is responsible for feature encoding of primary information which is coarse and time-invariant while the channel-pruned model enhances the learned representations with high-precision time-varing residual information. 
%Before discussing the technical details, we define the notations and the expressions used in this paper. 

%The former network plays a role as a backbone network while the latter encodes time-varying residual information.
%The former network plays a role as a primary network while the latter encodes fine-grained residual information.
%The proposed algorithm is composed of two parallel networks for learning accurate representations, but updates the residual network only for online learning to minimize run-time complexity.
%Contrary to the prior studies~\cite{jung2019learning, gong2019differentiable}, which adopt fully connected layers in full precision on top of quantized convolutional layers for stable online learning, 

For a given input image $A_0$, we compute a feature map $A_\textrm{conv}$ by applying a sequence of convolutions with auxiliary operations. 
The standard convolutional neural network (CNN) derives the feature map in the $i^\text{th}$ intermediate layer as follows:
%
\begin{equation}
A_{i} = \sigma(A_{i-1} * W_{i} ),
\end{equation}
%
where $W_i$ is the parameter of the $i^\text{th}$ convolution layer, $\sigma(\cdot)$ denotes a non-linear activation function and $*$ indicates the convolution operator. 
By representing the entire convolution layers as a feature extractor function $\mathtt{f}_\textrm{conv}(\cdot ; \cdot)$, the relationship between input and output activation is described as
%
\begin{equation} \label{formula:conv_layer}
    A_\textrm{conv} = A_{N_l}  = \mathtt{f}_\textrm{conv} (A_{0}; \mathcal{W}_\textrm{conv}),
\end{equation}
where $\mathcal{W}_\textrm{conv} = \{ W_1, ..., W_{N_l}\}$ is a collection of convolutional filters throughout the $N_l$ layers.
Contrary to the conventional CNNs, our framework utilizes two networks in parallel, a quantized network $\mathtt{f}^q (\cdot ; \cdot)$ and a channel-pruned network $\mathtt{f^p} (\cdot ; \cdot)$,
%Denote by $\mathcal{W}^q = \{ W^q_l \}_{l=1:N_l}$ and $\mathcal{W}^p = \{ W^p_l \}_{l=1:N_l}$ the $N_b$-bit quantized parameters of the backbone network and the channel-pruned parameters in the residual branch, respectively.
which generate outputs independently as 
%
\begin{align}
    A^\textrm{q} = \mathtt{f}^q(A_0; \mathcal{W}^\textrm{q}), ~~~ \mathcal{W}^\textrm{q}=\{ W_1^\textrm{q},...,W_{N_l}^\textrm{q} \}, \\
    A^\textrm{p} = \mathtt{f}^p(A_0; \mathcal{W}^\textrm{p}),  ~~~ \mathcal{W}^\textrm{p}=\{ W_1^\textrm{p},...,W_{N_l}^\textrm{p} \}.
\end{align}
Then, the proposed hybrid representation, $A^\textrm{h}$, is given by the sum of two outputs as follows:
%%%%%%%%
\begin{equation}
A^\textrm{h} = A^q + A^p \nonumber = \mathtt{f}^\textrm{q}(A_0; \mathcal{W}^q) + \mathtt{f}^\textrm{p}(A_0; \mathcal{W}^p). 
\end{equation}
%%%%%%%%
%
We can train prediction networks of arbitrary tasks coming after the feature extraction.
Note that the hybrid representation is also utilized on prediction networks; channel pruning is applied to all layers of the prediction networks while low-bit quantization is applied to the activation quantization partially.

\subsection{Low-Bit Quantization of Primary Network}
\label{sub:low-bit}
To maximize the benefit of the reduced precision network, 
we quantize both model parameters %, $\mathcal{W}_\textrm{conv} = \{W_{l}\}_{l=1:N_l}$, 
and feature activations %, $\mathcal{A} = \{A_l \}_{l=1:N_l}$, 
in all $N_l$ layers of the CNN backbone.
%We adopt the quantization method proposed in \cite{jung2019learning} except for the input of the first convolution layer and the output of the last convolution layer. 
We adopt the quantization method proposed in \cite{jung2019learning}. 
We also introduce the additional regularization loss terms to the quantized data for fast and stable training.
%In addition to the quantization algorithm,  we also introduce the additional regularization loss terms to the quantized data for fast and stable training.
%In the rest of this subsection, we describe the quantization method and normalization technique employed in our work.

\subsubsection{Weight Quantization}

The weight quantization function $Q_W^l(\cdot): w_l \rightarrow w^q_l$ is composed of the following two steps.
First, the weights are linearly transformed to $[-1,1]$ by the learnable parameters $\{ c^l_W, d^l_W\}$,  where each variable defines the center and the width of the quantization interval, respectively.
% First, the weights are linearly transformed to $[-1,1]$ by the learnable parameters $\{ c^l_W, d^l_W\}$, which define the center and the width of the quantization interval. 
Only the weights whose values are in the interval $[c_W^l-d_W^l, c_W^l+d_W^l]$ are quantized while the rests are clamped, which is formally given by
%
\begin{equation}
\hat{w}_{l} =
\begin{cases}
\mathtt{sign}(w_{l}) & \text{if $|w_{l}| > c^l_{W} + d^l_{W}$ } \\
0 & \text{if $|w_{l}| < c^l_{W} - d^l_{W}$ } \\
\mathtt{sign}(w_{l}) \cdot (\alpha^l_{W} |w_{l}| + \beta^l_{W}) & \text{otherwise},
%\texttt{sign}(w_{l}) \cdot (\alpha^l_{W} |w_{l}| + \beta^l_{W})^{\gamma^l_{W}} & \text{otherwise},
\end{cases}
\label{eq:quantization_w}
\end{equation}
%
where $\mathtt{sign}(\cdot) \in \{-1, 1\}$ indicates the sign of an input, $\alpha^l_{W} = 0.5/d^l_{W}$, and $\beta^l_{W}= -0.5 c^l_{W} / d^l_{W} + 0.5$. 
Second, the normalized weights are discretized by the element-wise rounding, $\mathtt{round}(\cdot)$, as $W^q_l = \mathtt{round}(\hat{W}_l \cdot (2^{N_b-1}-1))$, 
%%
%\begin{equation}
%W^q_l = \mathtt{round}(\hat{W}_l \cdot (2^{N_b-1}-1)),
%\label{eq:quantize_w}
%\end{equation}
%%
where $N_b$ is the given bit-width, and there is a $(2^{N_b}-1)$ distinguishable quantization levels. % Note that \eqref{eq:quantize_w} quantizes the absolute values of weights using $N_b-1$ bits and one bit is reserved for the sign of each weight.



%\ilchae{[Explanation of acitivation quantization]}
\subsubsection{Activation Quantization}
% The activation quantization function $Q_A^l(\cdot): a_l \rightarrow a^q_l$ also has two steps.
% First, all activations $a_l \in A_l$ in the $l^\text{th}$ layer are transformed to $\hat{a}_l \in \hat{A}_l$, which is in the range of $[0, 1]$ as in the following equation:
Similarly, the activation quantization function $Q_A^l(\cdot): a_l \rightarrow a^q_l$ also has two steps of transformation and round operation.
First, all activations $a_l \in A_l$ in the $l^\text{th}$ layer are transformed to be fallen into the range of $[0, 1]$ as in the following equation:

%
\begin{equation}
\hat{a}_l = 
\begin{cases}
1 & \text{if $a_l > c^l_{A} + d^l_{A}$ } \\
0 & \text{if $a_l < c^l_{A} - d^l_{A}$ } \\
\alpha^{l}_{A} A_l + \beta^{l}_{A} & \text{otherwise},
\end{cases}
\label{eq:quantization_a}
\end{equation}
%
where $\alpha^l_{A} = 0.5/d^l_{A}$ and $\beta^l_{A}= -0.5 c^l_{A} / d^l_{A} + 0.5$. The quantization interval is updated by backpropagation through the learnable parameters for its center ($c^l_A$) and width ($d^l_A$). 
Note that the activations assumes to be non-negative due to the ReLU function.  
%In other words, $[c^l_{A} - d^l_{A}, c^l_{A} + d^l_{A}]$ is transformed linearly to $[0, 1]$.
The final quantized output $A^q_l$ is obtained by applying the rounding function to the individual elements in $\hat{A}_l$, which is given by $A^q_l =  \mathtt{round}(\hat{A}_l \cdot (2^{N_b}-1))$.
%%
%\begin{equation}
%A^q_l =  \mathtt{round}(\hat{A}_l \cdot (2^{N_b}-1)).
%\label{eq:quantize}
%\end{equation}
%%
%We define whole matrix-wise transformation as $\mathtt{trans}^l_A() \textrm{ s.t. }  \hat{A}_l=\mathtt{trans}^l_A(A_l)$.
%

\subsubsection{Operation of Quantization Network}
% To reduce the computational cost, we apply both the activation and weight quantization at the same time during the convolution operation. 
%To reduce the computational cost of the neural network, both the weight quantization function $Q_W^l(\cdot)$ and the activation quantization function $Q_A^l(\cdot)$ are applied to the convolution layer.
%Specifically, the output from each convolutional layer is given by
The output from each convolutional layer is given by $A_{l+1} = \sigma (Q_A^l(A_l) * Q_W^{l+1}(W_{l+1}) ),$
%% 
%\begin{equation}
%A_{l+1} = \sigma (Q_A^l(A_l) * Q_W^{l+1}(W_{l+1}) ),
%\end{equation}
%
where standard convolution operation is replaced by a hardware-friendly fixed-point operation for additional acceleration.
By applying the quantization to the whole network, the representation of the final convolutional layer, denoted by $A^q$, is obtained by $A^q=\mathtt{f}^q(A_0; \mathcal{W}^q)$,
%%
%\begin{equation}
%A^q=\mathtt{f}^q(A_0; \mathcal{W}^q),
%\end{equation}
%
where $\mathtt{f}^q (\cdot ; \cdot)$ is the network with a joint quantization of weight and activation.
%Figure~\ref{fig:quantization} illustrates the framework of quantizing each layer's input activation.
%%%%%%%%%%%%%%%
\iffalse
\begin{figure}
	\centering
		\includegraphics[width=0.98\linewidth]{figs/quantization.pdf}
		\vspace{-0.1cm}
	\caption{Overall framework of quantizing $l^\textrm{th}$ layer's input activation. By observing input activation set $A_l$, we linearly transform the activations within quantization interval ($c^l_A - d^l_A,c^l_A + d^l_A$) to be locate in [0,1] (\textbf{Trans}). Note that the values lower than $c^l_A - d^l_A$ are pruned to 0 while the values upper than $c^l_A + d^l_A$ are clamped to 1. After that, we obtain quantized activations $A^q_l = \mathtt{round}(\hat{A}_l \cdot (2^N_b -1))$ (\textbf{Quantize}).} 
	\label{fig:quantization}
\end{figure} 
\fi
%%%%%%%%%%%%%%%%


\iffalse
\paragraph{Weight quantization.}
\textcolor{blue}{We convert all  model parameters in each convolutional layer within the range [0, 1] by a clipped transformation.
}
The original model parameters $w_l \in W_l$ are transformed to $\hat{w} \in \hat{W}_l$, which is in the range of $[-1, 1]$, by learning $(c^l_W, d^l_W, \gamma_W^l)$ and computing the following equation:
%
\begin{equation}
    \hat{w}_{l} =
        \begin{cases}
            \mathtt{sign}(w_{l}) & \text{if $|w_{l}| > c^l_{W} + d^l_{W}$ } \\
            0 & \text{if $|w_{l}| < c^l_{W} - d^l_{W}$ } \\
            \mathtt{sign}(w_{l}) \cdot (\alpha^l_{W} |w_{l}| + \beta^l_{W})^{\gamma^l_{W}} & \text{otherwise},
        \end{cases}
\label{eq:quantization_w}
\end{equation}
%
where $\alpha^l_{W} = 0.5/d^l_{W}$ and $\beta^l_{W}= -0.5 c^l_{W} / d^l_{W} + 0.5$.
The final quantized parameter, $W^q_l$  is obtained by applying the rounding function to the individual elements in $\hat{W}$, which is given by
%
\begin{equation}
W^q_l =  \frac{\mathtt{round}(\hat{W}_l \cdot (2^{N_b-1}-1))}{2^{N_b-1}-1}.
\label{eq:quantize_w}
\end{equation}
%


%\ilchae{[Explanation of acitivation quantization]}
\paragraph{Activation quantization.}
We convert all the activations in each convolutional layer within the range $[0, 1]$ by a clipped linear transformation.
Let $A_l$ be the output activation of the $l^\textrm{th}$ convolutional layer and $a_l$ be its single element.
Then, the transformation is given by learning the center and the width of the activation interval, denoted by $c^l_{A}$  and $d^l_{A}$, respectively, and applying the following equation:
%
\begin{equation}
    \hat{a}_l \equiv \mathtt{trans}_A^l(a_l) = 
            \begin{cases}
            1 & \text{if $a_l > c^l_{A} + d^l_{A}$ } \\
            0 & \text{if $a_l < c^l_{A} - d^l_{A}$ } \\
            \alpha^{l}_{A} A_l + \beta^{l}_{A} & \text{otherwise},
        \end{cases}
\label{eq:quantization_a}
\end{equation}
%
where $\alpha^l_{A} = 0.5/d^l_{A}$ and $\beta^l_{A}= -0.5 c^l_{A} / d^l_{A} + 0.5$.
In other words, $[c^l_{A} - d^l_{A}, c^l_{A} + d^l_{A}]$ is transformed linearly to $[0, 1]$.
The final quantization output, $A^q_l$ is given by applying the a rounding function, $\mathtt{round}(\cdot)$ to the individual elements in $\hat{A}_l$ as
%
\begin{equation}
A^q_l = \mathtt{quantize}(\hat{A_l}) = \frac{\mathtt{round}(\hat{A}_l \cdot (2^{N_b}-1))}{2^{N_b}-1},
\label{eq:quantize}
\end{equation}
%
where $N_b$ is the bit capacity and $\mathtt{quantize}(\cdot)$ denotes the quantization function.
%We define whole matrix-wise transformation as $\mathtt{trans}^l_A() \textrm{ s.t. }  \hat{A}_l=\mathtt{trans}^l_A(A_l)$.

\ilchae{Add figure that illustrate the steps of quantization}

The activation in each layer of a quantized network is given by 
\begin{align}
A^q_{l+1} &= \mathtt{quantize} ( \mathtt{trans}^l_A( \sigma (A^q_l * W^q_{l+1}) ) ), & l &= 0 \dots N_{l}-2 \\
A^q_{N_l} &= \sigma (A^q_{N_l-1} * W^q_{N_l}), & l &= N_l - 1,
\end{align}
%
where $\mathtt{quantize}(\cdot)$ and $\mathtt{trans}^l_A(\cdot)$ are defined in \eqref{eq:quantization_a} and \eqref{eq:quantize}, respectively, and $*$ denote the convolution operator.
The representation of the final convolutional layer, denoted by $A_\textrm{quant}$, is obtained by applying the quantization network, $\mathtt{f}_\textrm{quant}$, as follows:
%
\begin{equation}
A_\textrm{quant}=\mathtt{f}_\textrm{quant}(A_0; \mathcal{W}^q),
\end{equation}
where $ \mathcal{W}^q =  \{ W^q_l  \}_{l=1,,,N_l} $ is a set of quantized model parameters.
\fi

\subsubsection{Training Quantization Networks with Normalization}
We present our training technique for robust and stable quantization. 
In particular, we define a novel regularization loss for quantization, $\mathcal{L}_\textrm{quant}$, via proper normalization of weights and activations as $\mathcal{L}_\textrm{quant} = \mathcal{L}_\textrm{qW} + \mathcal{L}_\textrm{qA}$.
%%
%\begin{align}
%	\mathcal{L}_\textrm{quant} = \mathcal{L}_\textrm{qW} + \mathcal{L}_\textrm{qA}.
%\end{align}
%%
We discuss each of two loss terms in the following.

%%%%%%%%%%%%%%%
\iffalse
\begin{figure}
	\centering
		\includegraphics[width=0.95\linewidth]{figs/L_qw.pdf}
	\caption{Clipping model parameters using the learned interval leads to losing details in the quantized representations and makes the optimization procedure unstable. To alleviate the limitation, we propose a simple but effective regularizer, $\mathcal{L}_\textrm{qW}$,encouraging a majority of parameters to be located within a certain range.} 
	\label{fig:lqw}
\end{figure} 
\fi
%%%%%%%%%%%%%%%%

%\ilchae{[weight normalization with standard distribution]}
\paragraph{Weight normalization.}
Clipping model parameters using the learned interval $[c_W^l - d_W^l, c_W^l + d_W^l]$ leads to losing details in the quantized representations and makes the optimization procedure unstable.
%It turns out that the final accuracy is sensitive to the initialization of $(c^l_W, d^l_W, \gamma_W^l)$, which is aggravated when the quantization is based on lower bits\footnote{When we attempted the network quantization based on \cite{jung2019learning}, 5-bit quantization was much easier than 4-bit counterpart.}.
It turns out that the final accuracy is sensitive to the initialization of $\{c^l_W, d^l_W\}$, especially with a lower bit-width\footnote{When we tested network quantization based on \cite{jung2019learning}, 5-bit task was much easier than 4-bit counterpart.}.
To alleviate the limitation, we propose a simple but effective regularizer, $\mathcal{L}_\textrm{qW}(W_\textrm{conv})$, encouraging a majority of parameters to be located within a certain range, which is given by
%
\begin{align}
    \mathcal{L}_\textrm{qW}(\mathcal{W}_\textrm{conv}) = \sum^{N_l}_{i=1} \begin{pmatrix}\left(\mathtt{avg}({ \alpha^i_W |W_{i}| +\beta^i_W }) - \mu_0\right)^2 \nonumber \\  +\left(\mathtt{std}({  \alpha^i_W |W_{i} | + \beta^i_W })-\sigma_0\right)^2 \end{pmatrix} ,
\end{align}
%\ilchae{shoud fix the regularizer. Motivation(regularizing the range containing the most of parameters and activateion) is not changed.}
%
where $\mathtt{avg}(\cdot)$ and $\mathtt{std}(\cdot)$ denote mean and standard deviation of all entries in their input matrices, respectively, $| \cdot |$ returns an absolute value matrix of the same size to its input, and $(\mu_0, \sigma_0)$ are hyperparameters to define desirable mean and standard deviation values.
% By selecting the proper values in the range of $( 0,1 )$ for both $\mu_0$ and $\sigma_0$, the regularizer enforces model parameters to move into the range.
% By enforcing the distribution of model parameters using this regularizer, it is possible to identify more appropriate parameters ($c^l_W, d^l_W$) and train the network more efficiently and stably.
The proposed regularizer enforces the distribution of the transformed model parameters to be within the range of $( 0,1 )$, minimizing the loss of details inherent in clamping process.
This enables the quantized network to identify more appropriate parameters ($c^l_W, d^l_W$) and optimize with more stability.

%Figure~\ref{fig:lqw} illustrate the effect of the weight normalization briefly.


\paragraph{Activation normalization.}
\label{paragraph:act_norm}
Clipping activations outside of the interval $[c^l_\textrm{A}-d^l_\textrm{A}, c^l_\textrm{A}+d^l_\textrm{A}]$ incurs critical information loss in practice.
%To mitigate this issue, we employ a similar technique with weight normalization and define the following regularization loss term $\mathcal{L}_\textrm{qA}$:
To mitigate this issue, we define the following regularization loss term $\mathcal{L}_\textrm{qA}$:
%
\begin{align}
%    \mathcal{L}_\textrm{qA}(A^\textrm{bn}) = \sum^{N_l}_{i=1} \left[ \mathtt{avg}(A_i^\textrm{bn}) + 2 \cdot \mathtt{std}(A_i^\textrm{bn}) - \mathtt{UB} \right]_{+} \nonumber   +  \left[ \sigma_i - \mathtt{std}(A_i^\textrm{bn}) \right]_{+} +  \left[ \mu_i - \mathtt{avg}(A_i^\textrm{bn}) \right]_{+},
    %\mathcal{L}_\textrm{qA} & (A^\textrm{bn}) =  \\
    %& \sum^{N_l}_{i=1} \left[ \mathtt{avg}(A_i^\textrm{bn}) + 2 \cdot \mathtt{std}(A_i^\textrm{bn}) - (c^l_\textrm{A}+d^l_\textrm{A}) \right]_{+} \hspace{-0.1cm}  +  \left[ \sigma_i - \mathtt{std}(A_i^\textrm{bn}) \right]_{+} \hspace{-0.1cm} + \left[ \mu_i - \mathtt{avg}(A_i^\textrm{bn}) \right]_{+}, \nonumber
    \mathcal{L}_\textrm{qA} & (A^\textrm{bn}) =  \sum^{N_l}_{i=1}\{ \left[ \mathtt{avg}(A_i^\textrm{bn}) + 2 \cdot \mathtt{std}(A_i^\textrm{bn}) - (c^l_\textrm{A}+d^l_\textrm{A}) \right]_{+}  \nonumber \\ &+  \left[ \sigma_i - \mathtt{std}(A_i^\textrm{bn}) \right]_{+}  + \left[ \mu_i - \mathtt{avg}(A_i^\textrm{bn}) \right]_{+}\}, 
\end{align}
%
where $A^\textrm{bn}=\{  A_i^\textrm{bn}  \}_{i=1}^{N_l}$ is a set of activations after batch normalization and $\left[ \cdot \right]_+$ denotes the ReLU function.
Note that $\sigma_i$ and $\mu_i$ are determined by combination of current quantization interval parameters ($c^l_A, d^l_A$).
Assuming that the activation $A_i^\textrm{bn}$ follows a Gaussian distribution, the regularization loss enforces the activations larger than the mean of the Gaussian and lower than $\mathtt{avg}(A^\textrm{bn}_i)+2\cdot \mathtt{std}(A^\textrm{bn}_i)$ to be within the active range.
Statistically speaking, it implies that almost 96$\%$ of positive values are trained to be located in the active range.
%Figure~\ref{fig:lqa} illustrate the effect of the activation normalization briefly.
%%%%%%%%%%%%%%%
\iffalse
\begin{figure}
	\centering
		\includegraphics[width=0.95\linewidth]{figs/L_qa.pdf}
	\caption{Clipping activations outside of the interval incurs critical information loss in practice. To mitigate this issue, we employ a similar technique with weight normalization and define the regularization loss term $\mathcal{L}_\textrm{qA}$.} 
	\label{fig:lqa}
\end{figure}
\fi 
%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
	\centering
		\includegraphics[width=0.9\linewidth]{figs/framework.pdf}
		%\vspace{-0.1cm}
	\caption{Overall framework of our algorithm. We train hybrid representation for both low-bit quantized network ($\mathtt{f}^q$) and lightweight full precision network ($\mathtt{f}^p$) on pretraining time while only light weight network is fine-tuned in test phase.
	Red arrow denotes the gradient backpropagation of full precision network in online model update and pretraining while blue arrow denotes the backpropagation in pretraining. 
%Note that $\mathcal{L}_\textrm{track}$ denotes the original objective of baseline trackers.
}
	\label{fig:overall_framework}
	\vspace{-0.4cm}
\end{figure*} 
%%%%%%%%%%%%%%%%%%%

\subsection{Channel Pruning of Residual Network}
\label{sub:channel}

%\ilchae{[Explanation of gumbel softmax application to model channel pruning]}
We propose a stochastic channel pruning algorithm using a Gumbel-softmax trick to generate discrete mask samples from the model with a continuous output space.
Our algorithm learns a set of channel selection probability vectors, $\{ \mathbf{b}_1, ..., \mathbf{b}_{N_{l}}\}$, in each layer, where $\mathbf{b}_l$ indicates which channel is likely to be sampled in the $l^\textrm{th}$ layer.
%Note that we employ channel pruning algorithm for all $N_{pl}$ layers of whole model including $N_l$ layers of backbone CNN.
By employing the Gumbel-softmax trick introduced in ~\cite{jang2016categorical}, $\mathbf{b}_l$ generates discrete channel selection mask $\mathbf{M}_{l}$ as follows:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\label{formula:pruning}
    %\begin{matrix}
\bar{\mathbf{M}}_l[i] & = \frac{\mathtt{exp}\left( \frac{g_i + \mathtt{log} (\mathbf{b}_l[i])}{\tau} \right) }{ \mathtt{exp} \left( \frac{g_i + \mathtt{log} (\mathbf{b}_l[i])}{\tau} \right) + \mathtt{exp} \left( \frac{g_i + \mathtt{log}(1- \mathbf{b}_l[i])}{\tau} \right) }, \nonumber \\
\mathbf{M}_l[i] & = \mathtt{round}(\bar{\mathbf{M}}_l[i]) , 
    %\end{matrix}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $g_i$ represents a random noise sample from Gumbel distribution, and $\tau$ denotes a temperature.
%where $g_i$ represents a random noise sample from Gumbel distribution, $\mathtt{Gumbel}(0,1)$, and $\tau$ denotes a temperature.
Similarly to \cite{jang2016categorical}, we apply the straight-through Gumbel estimator for gradient approximation in backpropagation.
In the forward pass of training, we apply the pruning mask $M_{l}$ to the output activation  $A^p_l$ in the $l^\textrm{th}$ layer, which is given by
%
\begin{equation}
A^p_{l} = \sigma ( A^p_{l-1} * W^p_{l} ) \odot \mathbf{M}_{l},  \quad l =1 \dots N_{l}
\end{equation}
%
where $\odot$ denotes an channel-wise multiplication.
%where $l =1 \dots N_{pl}$ and $\odot$ denotes an channel-wise multiplication.
Then, the representation of the final convolution layer is obtained by applying the channel pruning network $\mathtt{f}^p(\cdot ; \cdot)$, as follows: $A^p =  \mathtt{f}^p(A_0; \mathcal{W}^p)$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{align}
%	A^p &=  \mathtt{f}^p(A_0; \mathcal{W}^p),
%\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%where $ \mathcal{W}^p = \{ W^p_l \}_{l=1}^{N_{pl}}$ is the set of convolution parameters in the pruned network.
Note that a channel with a selection probability lower than the threshold is removed at testing.
For training, the channel selection probabilities $ \{ \mathbf{b}_l \}^{N_{l}}_{l=1}$ are learned by minimizing the following loss term $\mathcal{L}_\textrm{prune}= \sum^{N_{l}}_{l=1} ||\mathbf{M}_{l}||_1$, where the number of active channels is penalized.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{align}
 %   \mathcal{L}_\textrm{prune} = \sum^{N_{pl}}_{l=1} ||\mathbf{M}_{l}||_1.
 %   %\mathcal{L}_\textrm{pW} = \sum^{N_l}_{l=2} ||\mathbf{M}_{l}||_1.
%\end{align}

